On the Capacity of Multi-Hop Wireless Networks with Partial Network Knowledge

In large wireless networks, acquiring full network state information is typically infeasible. Hence, nodes need to flow the information and manage the interference based on partial information about the network. In this paper, we consider multi-hop wireless networks and assume that each source only knows the channel gains that are on the routes from itself to other destinations in the network. We develop several distributed strategies to manage the interference among the users and prove their optimality in maximizing the achievable normalized sum-rate for some classes of networks.

==> conclusion.tex <==
In this paper, we developed a new model for partial netwrok knowledge in acyclic wireless networks. Different schemes were studied and their performances were examined in several cases, in terms of the normalized sum-capacity. Deep connections between network topology, normalized sum-capacity and the achievability strategies were noticed, and we saw several motivating results. One of the important future directions is to extend our results to Gaussian networks.

In this paper, we have only studied cases with $1$-local view, a major direction is to figure out how normalized sum-capacity increases as nodes learn more and more about the network. Moreover, we have considered the case that the nodes know the network-connectivity globally, but the actual values of the channel gains are only known for a subset of routes. An appealing extension in this case, would be to understand the effects of local knowledge about network connectivity on the capacity and develop distributed strategies to optimally route information with partial knowledge about network connectivity. It is also desired to develop scalable network coding strategies that only rely on local network information. As mentioned before, the very idea of developing fundamental information-theorectic based foundations for networks with partial information at nodes is in its beginning stages and as a result, there are many salient directions to work on.
%that inspired the promising future of this area.

==> future.tex <==
As mentioned before, the very idea of developing fundamental information-theorectic based foundations for networks with partial information at nodes is in its beginning stages and as a result, there are many salient directions to work on. We list a couple of broad directions for future work.

{\bf Multi-Flow Multi-Layer Network Coding with Partial Information}: It is a well established fact that network coding is an effective technique to increase the spectral efficiency of the networks. However, a major problem is how to effectively exploit network coding with partial network state information. The problem becomes really challenging when we are dealing with multi-commodity flows, such as the one depicted in Figure \ref{kdcyclic}. We believe that there is a deep connection between network geometry and optimal schemes with partial knowledge. Therefore, one of the future directions is to develop scalable network coding strategies that only rely on local network information.

{\bf Determining the Impact of Incomplete Network Topology}:  So far, we have considered the case that the nodes know the network-connectivity globally, but the actual values of the channel gains are only known for a subset of routes. An appealing extension in this case, would be to understand the effects of local knowledge about network connectivity on the capacity and develop distributed strategies to optimally route information with partial knowledge about network connectivity.

{\bf Extending the result to $h$-local view, $h > 1$,}: In this paper, we have only studied cases with $1$-local view, a major direction is to figure out how normalized sum-capacity increases as nodes learn more and more about the network.

{\bf Determining the Impact of Inaccurate Network State Estimation}: We have considered cases where each node has a perfect knowledge about part of the network, but has no information about the rest (except for topology). An interesting direction is to incorporate error in network estimations in our results and study its effects on network sum-capacity.

{\bf Deriving the Connections between Network Complexity and Network Capacity}: In our preliminary results for multi-layer networks, we have seen examples that prove the strong connections between the complexity of network topology (e.g., maximum degree of the nodes, etc) and network capacity with partial information. It is desired to derive exact connections between the complexity of network topology and network capacity with partial information in more general networks.

{\bf Gaussian Wireless Networks}: In this paper, we considered the linear deterministic model for the channels in the netwrok, one of the next steps is to generalize our results to Gaussian model.

==> intro.tex <==
One of the key challenges in the design of wireless networks is optimizing system efficiency while the network is constantly in flux. To manage system resources efficiently, it is crucial to keep track of the state of the network and determine what resources are actually available.  However, in large wireless networks, keeping track of the state for making optimal decisions is typically infeasible. Thus, in the absence of centralization of network state information, nodes have limited local view of the network and make distributed decisions, which are based on their own local view of the network. The key question then, is how do optimal distributed decisions perform in comparison to the optimal decisions when full network state information is available at all nodes.

All wireless networks (eg. 2G/3G, WiFi, WiMax Bluetooth, ZigBee) rely on a host of distributed coordination protocols for their operation.
%Coordination mechanisms operate at multiple time-scales, like symbol time-scale physical layer training and pilots~\cite{Rappaport:1996aa},  packet time-scale medium access protocols~\cite{Wu:2008aa,al:2009aa} and scheduling~\cite{Pantelidou:2010aa},  and mobility time-scale routing protocols~\cite{Tonguz:2006aa}.
The numerous protocol innovations have led to many practical advances in deployed networks. However, there is very little work in understanding the fundamental limits for distributed protocols~\cite{Gallager,Ephremides}.

A systematic study to understand the role of limited network knowledge, was first initiated in \cite{messageisit,messageit} for single-layer networks, where the authors used a message-passing abstraction of network protocols to formalize the notion of limited network view at each node in the form of number of message rounds; each message round adds two extra hops of channel information at each source. The key result was that distributed decisions can be either sum-rate optimal or can be arbitrarily worse than the global-information sum-capacity.

This result was further strengthened for arbitrary $k$-user single-layer interference network in \cite{aas09allerton,VaneetISIT,VaneetIT}, where the authors proposed a new metric, normalized sum-capacity, to measure the performance of distributed decisions. Further,  the authors computed the capacity of distributed decisions for several network topologies with one-hop and two-hop network information at each source. In this paper, we characterize the next major step in understanding the performance of distributed decisions for general acyclic linear deterministic networks \cite{ADTJ10}.

In single-layer networks, the main challenge is to manage the interference among the sources with partial network information. However, in more general networks, we face an additional complication - the relaying of information with partial network information in addition to managing interference at all nodes. While the hop-count model of \cite{VaneetIT} can still be used to quantify partial network-state information, we will develop a more scalable model for general acyclic networks in this paper, which is based on the knowledge about the routes in the network. The motivation for this model is that in general networks, coordination protocols like routing, aim to discover source-destination routes in the network. Hence, a more suitable quanta for network-state information is the number of such end-to-end routes that are known at the nodes.

Our results are three-fold. First, as mentioned we will develop a more scalable model for general acyclic networks in this paper. Second, we develop new strategies that can be used with this local knowledge, and third, we prove the optimality of these strategies for a variety of networks. 

In this paper, we will consider the case where each source has full information about network topology, as well as full information about the routes from itself to all the destinations. Each node (which is not a source), has the union of the information of all those sources that have a route to it. This model of partial information will be formally defined in Section~\ref{localview}. We will start by a natural extension of Maximum Independent Set (MIS) scheduling~\cite{aas09allerton,VaneetIT}, called the Maximum Independent Route (MIR) scheduling and we notice that it fails to perform optimally in many cases. We will remove a main limitation of MIR scheduling, and through this, we develop the Maximum Independent Link (MIL) scheduling and we prove its optimality for a class of networks, namely $k \times 2 \times k$ networks. We will face an interesting example, that shows the requirement of network coding at relays. This motivates us to consider a broader class of networks and strategies.

The rest of the paper is organized as follows. In section \ref{problem}, we will introduce our network model and the new model to capture partial network knowledge. Section \ref{background} is dedicated to a brief overview of the results for single-layer networks. In Section~\ref{strategies}, we describe our main results including the achievability schemes. We introduce upper bounds on the performance of distributed decisions based on local network knowledge in Section~\ref{upper}. %Motivating directions will be discussed in section \ref{future}.
Finally, Section~\ref{conclusion} concludes the paper and presents some future directions.

==> problem.tex <==
In this section, we first introduce our system and network models. We will then define the our model of local view in the network. Finally, we present the definitions of \emph{normalized sum-rate} and \emph{normalized sum-capacity}, which will be used extensively in this paper.

==> strategies.tex <==
In this section, we assume that the local view available at the transmitters is $1$-round local view and the topology is known globally. As discussed in section \ref{problem} excluding transmitters, each node has the union of the local view of all the transmitters that have at least a path to it.  We will study different transmission strategies alongside several different topologies. Through these examples, we notice the deep connections between network geometry, partial information and the normalized sum-capacity.
